The Mythos of Model Interpretability

Supervised machine learning models boast remarkable predictive capabilities. But can you trust your model? Will it work in deployment? What else can it tell you about the world? We want models to be not only good, but interpretable. And yet the task of interpretation appears underspecified. Papers provide diverse and sometimes non-overlapping motivations for interpretability, and offer myriad notions of what attributes render models interpretable. Despite this ambiguity, many papers proclaim interpretability axiomatically, absent further explanation. In this paper, we seek to refine the discourse on interpretability. First, we examine the motivations underlying interest in interpretability, finding them to be diverse and occasionally discordant. Then, we address model properties and techniques thought to confer interpretability, identifying transparency to humans and post-hoc explanations as competing notions. Throughout, we discuss the feasibility and desirability of different notions, and question the oft-made assertions that linear models are interpretable and that deep neural networks are not.

==> linear_vs_deep.tex <==
With these definitions, we now revisit 
the axiomatic claim that linear models are interpretable,
while deep neural networks are not.
For the subjective definition of \emph{understandability},
the question can only be addressed empirically (by human subjects studies),
or by fundamentally understanding the mechanism by which the human arbiters operate.
The popularity of the claim of that linear models exhibit superior interpretability
as compared to deep neural networks,
points to a subjective preference.
However, this may be subject to change 
as compelling post-hoc interpretations emerge for deep neural networks.
By this notion of interpretability, 
humans too be may be interpretable.

With respect to the \emph{simulatability} characterization, 
only models with low computational complexity are interpretable.
For a human to work through the decision process step by step, neither linear models with high dimensionality, not modern neural networks could be considered interpretable. Clearly, humans are not presently simulatably interpretable as we possess neither the computational power to simulate another human's brain nor a method to determine what precisely those computations might be.
Practically, 
linear models appear to have a distinct advantage over deep methods,
both because they tend generally to require fewer parameters and less computation,
and also because methods exist for inducing sparsity,
which significantly lowers the inference complexity 
to the number of nonzero parameters, 
rather than the total number of features.

Finally, with respect to \emph{decomposabity},
linear models exhibit a clear advantage. 
So long as the input features are themselves symbolically meaningful,
the corresponding parameters in a linear model each admit an intuitive description.
At present, we know of no method by which each individual parameter in a deep neural network,
or by which any neuron or synapse in a human brain
could be so conveniently described.
However, the weights learned by a linear model can be fickle with respect to feature selection.
The addition or deletion of a small number of features from a linear model may yield similar predictive accuracy and yet a vastly different interpretation.

Assessing the ability of any supervised learning model 
to shed light on causal relationships seems fraught.
At present linear models appear 
to more obviously suited to mining direct relationships 
between inputs and outputs.
However, newer methods for interpreting neural networks,
such as computing saliency maps % citation goes here
over the input, might prove similarly useful for hypothesis generation.

The issue of generalization is similarly difficult to address formally.
The example of detecting spurious hypotheses unlikely to generalize to the real-world for pneumonia risk given by \citet{caruanaintelligible} shows a compelling case where linear models admit analysis that current models deep learning models do not.
However, it's unclear that manual inspection of linear models can uncover all such spurious associations. 
Because the linear model learns associations and not causal relationships, an implausible mapping from an omitted variable may be encoded subtly via the many correlated variables represented in the model.

Finally, we consider the capacity of each model to produce extra useful information, absent any demands on understandability.
For linear models, the only useful information resides in the values of the weights, one per feature. 
However deep learning is especially amenable to post-hoc interpretation.
In addition to the value of the parameters,
we can plot saliency maps by backpropagating loss with respect to the input \cite{wang2015dueling}.
Additionally the hierarchical representations learned by a deep neural network have proven broadly useful,
both for predictions on related tasks,
and for mapping model states onto text descriptions.

==> sections/acknowledgments.tex <==
Thanks to Charles Elkan, Julian McAuley, Maggie Makar, David Kale, Been Kim, Lihong Li, Rich Caruana, Sepp Hochreiter, Daniel Fried, and Jack Berkowitz, for helpful conversations and critical feedback.
